What are the characteristics of highly-selected packages? A case study on the npm ecosystem

With the popularity of software ecosystems, the number of open source components (known as packages) has grown rapidly. Identifying high-quality and well-maintained packages from a large pool of packages to depend on is a basic and important problem, as it is beneficial for various applications, such as package recommendation and package search. However, no systematic and comprehensive work focuses on addressing this problem except in online discussions or informal literature and interviews. To fill this gap, in this paper, we conducted a mixed qualitative and quantitative analysis to understand how developers identify and select relevant open source packages. In particular, we started by surveying 118 JavaScript developers from the npm ecosystem to qualitatively understand the factors that make a package to be highly-selected within the npm ecosystem. The survey results showed that JavaScript developers believe that highly-selected packages are well-documented, receive a high number of stars on GitHub, have a large number of downloads, and do not suffer from vulnerabilities. Then, we conducted an experiment to quantitatively validate the developers' perception of the factors that make a highly-selected package. In this analysis, we collected and mined historical data from 2,527 packages divided into highly-selected and not highly-selected packages. For each package in the dataset, we collected quantitative data to present the factors studied in the developers' survey. Next, we used regression analysis to quantitatively investigate which of the studied factors are the most important. Our regression analysis complements our survey results about highly-selected packages. In particular, the results showed that highly-selected packages tend to be correlated by the number of downloads, stars, and how large the package's readme file is.

==> ExtraAnalysis.tex <==








==> Table_Regression_Modeling_Downloads.tex <==
\begin{tabular} {l|l|r|rl} %
	\hline
	\multirow{2}{*}{\textbf{Factors}} & \multirow{2}{*}{\textbf{D.f}} & \multirow{2}{*}{\textbf{$\textrm{Wald }\chi^{2}$}} & \multirow{2}{*}{\textbf{$p\textrm{-value}$}} & \multirow{2}{*}{\textbf{}} \\
	                                  &                               &                                            &                                   &                            \\  \hline \hline


Contributors       &1  &0.1620  &0.6873528 &   \\
Stars              &1 &16.0649  &6.121e-05 &***\\
Dependencies       &1 &13.2742  &0.0002691 &***\\
License            &1 &13.5673  &0.0002302 &***\\
Documentations     &1  &3.7919  &0.0514998 &.  \\
Build\_status       &1  &0.9196  &0.3375876 &   \\
Vulnerabilities    &1 &14.7413  &0.0001233 &***\\
Badges             &1  &7.2789  &0.0069767 &** \\
Website            &1  &5.6566  &0.0173898 &*  \\
Test\_code          &1 &30.6388  &3.108e-08 &***\\
Release            &1  &0.7920  &0.3734827 &   \\
Closed\_issue       &1  &5.5357  &0.0186328 &*  \\
Usage              &1  &3.7945  &0.0514204 &.  \\
Commits\_frequency  &1  &2.7220  &0.0989716 &. \\  
	
	
	\hline
	
	
	
	
	\multicolumn{5}{l}{\footnotesize{Signif. codes:  0 `***' 0.001 `**' 0.01 `*' 0.05 `.' 0.1 ` ' 1 }}                                                                              \\
\end{tabular}


==> Table_Regression_Modeling_lifetime.tex <==
\begin{tabular} {l|rrl|c}
	\toprule
	\textbf{Factors}  & \textbf{$\textrm{Wald }\chi^{2}$} & \multicolumn{2}{l|}{\textbf{$p\textrm{-value}$}} & \textbf{Shift}                 \\ \midrule
	Downloads         & 60.66                             & 0.000                                            & ***            & -             \\
	Badges            & 16.83                             & 0.000                                            & ***            & $\uparrow3$   \\
	Closed Issue      & 16.65                             & 0.000                                            & ***            & -             \\
	Stars             & 15.83                             & 0.000                                            & ***            & $\downarrow2$ \\
	Vulnerabilities   & 12.63                             & 0.000                                            & ***            & $\downarrow1$ \\
	Dependencies      & 8.94                              & 0.003                                            & **             & $\uparrow1$   \\
	Build Status      & 6.98                              & 0.008                                            & **             & $\uparrow1$   \\
	Documentation     & 6.80                              & 0.009                                            & **             & $\downarrow2$ \\
	Contributors      & 2.92                              & 0.087                                            & .              & $\uparrow1$   \\
	Test Code         & 2.91                              & 0.089                                            & .              & $\downarrow2$ \\
	Commits Frequency & 1.90                              & 0.168                                            &                & -             \\
	Usage             & 1.54                              & 0.214                                            &                & $\uparrow2$   \\
	License           & 1.53                              & 0.217                                            &                & -             \\
	Release           & 1.28                              & 0.257                                            &                & $\downarrow2$ \\
	Website           & 0.00                              & 0.954                                            &                & -             \\
	\bottomrule
	\multicolumn{5}{l}{\multirow{2}{*}{\footnotesize{Signif. codes:  0 `***' 0.001 `**' 0.01 `*' 0.05 `.' 0.1 `~' 1 }}}                       \\
\end{tabular}

